Generalized PINN-Based Inverse Estimation of Spatially Varying Heat Transfer Coefficients with Transfer Learning

This study investigates generalized boundary representations and transfer learning for physics-informed neural-network (PINN) estimation of spatially varying convective heat transfer coefficients (HTCs) in jet impingement cooling. Piecewise-linear (PWL) and neural-network boundary estimators are inferred from transient interior-temperature measurements and evaluated against CFD-CHT reference HTC profiles at Reynolds numbers of 5000, 10000 and 15000. A discrete Adjoint-FEM formulation with gradient regularization based on the $H^1$-seminorm provides an independent inverse-method comparison. Transfer learning is investigated under two source-target conditions: transfer between noise levels at the same Reynolds number, and transfer from a controlled Gaussian-profile problem to CFD-CHT-derived target problems at different Reynolds numbers. For the representative Re = 5000 target with 5% measurement noise, quadratic, PWL, and neural-network PINNs achieve relative HTC-profile errors of 5.08, 5.31 and 5.19%, respectively, while generalized representations reduce the error for the Re = 15000 target from 16.76% for the quadratic PINN to 14.41% and 14.46%. Transfer learning reduces target-training time by 57.86-81.71% for fixed-Reynolds-number transfer and by 50.59-84.94% for Gaussian-to-CHT transfer. Its effect on reconstruction accuracy is target dependent: fixed-profile PWL transfer remains within 0.30 percentage points of scratch training, whereas Gaussian-to-CHT transfer produces differences of 0.10-1.52 percentage points across targets and representations. These results demonstrate that generalized PINN representations can accommodate spatially varying HTC profiles without a prescribed quadratic form, while transfer learning can substantially reduce target-training cost for repeated inverse estimation, with the resulting reconstruction accuracy depending on source-target compatibility.

==> Figures/convergence_pgfplots_macros.tex <==
\pgfplotsset{
  conv axis/.style={
    grid=major,
    major grid style={draw=gray!35, line width=0.35pt},
    tick align=outside,
    tick style={black, line width=0.5pt},
    axis line style={black},
    line width=0.85pt,
    label style={font=\small},
    tick label style={font=\small},
    title style={font=\normalsize, yshift=2pt},
    legend style={
      draw=gray!55,
      fill=white,
      fill opacity=0.96,
      text opacity=1,
      rounded corners=1pt,
      font=\footnotesize,
    },
    legend cell align=left,
    ymode=log,
    log basis y=10,
    xlabel={Iteration},
    ylabel={Total loss},
    unbounded coords=discard,
  },
  convScratchTrain/.style={color=blue!80!black, line width=1.15pt, mark=none},
  convScratchTest/.style={color=red!80!black, line width=1.15pt, mark=none},
  convFTTrain/.style={color=green!50!black, line width=1.15pt, mark=none},
  convFTTest/.style={color=orange!90!black, line width=1.15pt, mark=none},
  convTLTrain/.style={color=violet!85!black, line width=1.15pt, mark=none},
  convTLTest/.style={color=magenta!60!black, line width=1.15pt, mark=none},
  convTLGaussTrain/.style={color=teal!75!black, line width=1.15pt, mark=none},
  convTLGaussTest/.style={color=brown!85!black, line width=1.15pt, mark=none},
  convNNTrain/.style={color=black, line width=1.15pt, mark=none},
  convNNTest/.style={color=pink!80!black, line width=1.15pt, mark=none},
  convTrain/.style={solid},
  convTest/.style={densely dashed},
  convNoiseFree/.style={
    color=black,
    line width=1.2pt,
    densely dashed,
    mark=none,
  },
  convNoiseFive/.style={
    color=blue!75!black,
    line width=1.2pt,
    densely dashed,
    mark=none,
  },
  convNoiseTen/.style={
    color=red!75!black,
    line width=1.2pt,
    densely dashed,
    mark=none,
  },
  selected loss axis/.style={
    grid=major,
    major grid style={draw=gray!30, line width=0.3pt},
    tick align=outside,
    tick style={black, line width=0.45pt},
    axis line style={black},
    line width=0.85pt,
    label style={font=\small},
    tick label style={font=\scriptsize},
    title style={font=\small, yshift=1pt},
    ymode=log,
    log basis y=10,
    xlabel={Training iteration ($\times 10^3$)},
    ylabel={Total PINN loss},
    unbounded coords=discard,
  },
  selected adjoint axis/.style={
    grid=major,
    major grid style={draw=gray!30, line width=0.3pt},
    tick align=outside,
    tick style={black, line width=0.45pt},
    axis line style={black},
    line width=0.85pt,
    label style={font=\small},
    tick label style={font=\scriptsize},
    title style={font=\small, yshift=1pt},
    xlabel={Objective evaluation},
    ylabel={Adjoint objective $J$},
    unbounded coords=discard,
  },
  selectedScratchTrain/.style={color=blue!75!black, line width=1.0pt, solid, mark=none},
  selectedScratchTest/.style={color=orange!90!black, line width=1.0pt, densely dashed, mark=none},
  selectedTLTrain/.style={color=green!50!black, line width=1.1pt, solid, mark=none},
  selectedTLTest/.style={color=magenta!70!black, line width=1.1pt, densely dashed, mark=none},
  selectedTL/.style={line width=1.1pt, mark=none},
  selectedScratch/.style={color=blue!75!black, line width=1.1pt, solid, mark=*},
  selectedTransfer/.style={color=green!50!black, line width=1.1pt, solid, mark=square*},
  selectedScratchStop/.style={color=blue!75!black, only marks, mark=star, mark size=3.3pt, forget plot},
  selectedTransferStop/.style={color=green!50!black, only marks, mark=star, mark size=3.3pt, forget plot},
  selectedTLStop/.style={color=red!75!black, only marks, mark=star, mark size=3.3pt, forget plot},
  selectedAdjointStop/.style={color=red!75!black, only marks, mark=star, mark size=3.3pt, forget plot},
  selectedTrain/.style={color=blue!75!black, solid},
  selectedTest/.style={color=orange!90!black, densely dashed},
  selectedCurveA/.style={color=blue!75!black, line width=1.1pt, mark=none},
  selectedCurveB/.style={color=orange!90!black, line width=1.1pt, mark=none},
  selectedCurveC/.style={color=green!50!black, line width=1.1pt, mark=none},
}

\newcommand{\MonitoredLossAddSeries}[6]{%
  \addplot+[#6] table[
    col sep=comma,
    x expr=\thisrow{iteration}/1000,
    y=loss_total,
    restrict expr to domain={\thisrow{#2}}{#3:#3},
    restrict expr to domain={\thisrow{representation_id}}{#4:#4},
    restrict expr to domain={\thisrow{method_id}}{#5:#5},
  ] {#1};
}

\newcommand{\MonitoredLossAddStop}[6]{%
  \addplot+[#6] table[
    col sep=comma,
    x expr=\thisrow{iteration}/1000,
    y=loss_total,
    restrict expr to domain={\thisrow{#2}}{#3:#3},
    restrict expr to domain={\thisrow{representation_id}}{#4:#4},
    restrict expr to domain={\thisrow{method_id}}{#5:#5},
    restrict expr to domain={\thisrow{is_terminal}}{1:1},
  ] {#1};
}

\newcommand{\CommonLossAddSeries}[7]{%
  \addplot+[#7] table[
    col sep=comma,
    x expr=\thisrow{iteration}/1000,
    y=common_loss,
    restrict expr to domain={\thisrow{#2}}{#3:#3},
    restrict expr to domain={\thisrow{representation_id}}{#4:#4},
    restrict expr to domain={\thisrow{method_id}}{#5:#5},
    restrict expr to domain={\thisrow{split_id}}{#6:#6},
  ] {#1};
}

\newcommand{\SelectedAdjointAddSeries}[5]{%
  \addplot+[#5] table[
    col sep=comma,
    x=iteration,
    y=J,
    restrict expr to domain={\thisrow{group_id}}{#2:#2},
    restrict expr to domain={\thisrow{curve_id}}{#3:#3},
  ] {#1};
  \addlegendentry{#4}
}

\newcommand{\SelectedAdjointAddSeriesNoLegend}[4]{%
  \addplot+[#4,forget plot] table[
    col sep=comma,
    x=iteration,
    y=J,
    restrict expr to domain={\thisrow{group_id}}{#2:#2},
    restrict expr to domain={\thisrow{curve_id}}{#3:#3},
  ] {#1};
}

\newcommand{\SelectedAdjointAddStop}[4]{%
  \addplot+[#4] table[
    col sep=comma,
    x=iteration,
    y=J,
    restrict expr to domain={\thisrow{group_id}}{#2:#2},
    restrict expr to domain={\thisrow{curve_id}}{#3:#3},
    restrict expr to domain={\thisrow{is_terminal}}{1:1},
  ] {#1};
}

\newcommand{\SelectedLegendLine}[1]{%
  \tikzset{external/export next=false}%
  \tikz[baseline=-0.5ex]{\draw[#1] (0,0)--(0.7,0);}%
}

\newcommand{\PINNAddSeries}[5]{%
  \addplot+[
    #5,
  ] table[
    col sep=comma,
    x=iteration,
    y=total_loss,
    restrict expr to domain={\thisrow{noise}}{#2:#2},
    restrict expr to domain={\thisrow{methodid}}{#3:#3},
    restrict expr to domain={\thisrow{splitid}}{#4:#4},
  ] {#1};
}

\newcommand{\AdjointAddSeries}[3]{%
  \addplot+[
    #3,
  ] table[
    col sep=comma,
    x=objective_evaluation,
    y=J,
    restrict expr to domain={\thisrow{noise}}{#2:#2},
  ] {#1};
}

\newcommand{\ConvLegendItem}[2]{%
  \addlegendimage{#1}
  \addlegendentry{#2}
}

\newcommand{\ConvLegend}[2]{%
  \begin{tikzpicture}
    \begin{axis}[
      hide axis,
      xmin=0,
      xmax=1,
      ymin=0,
      ymax=1,
      legend columns=#1,
      legend style={
        draw=gray!55,
        fill=white,
        fill opacity=0.96,
        text opacity=1,
        rounded corners=1pt,
        font=\footnotesize,
        /tikz/every even column/.append style={column sep=0.8em},
      },
    ]
#2
    \end{axis}
  \end{tikzpicture}
}

\newcommand{\PINNConvergencePanel}[3]{%
  \begin{tikzpicture}
    \begin{groupplot}[
      group style={
        group size=1 by 3,
        vertical sep=1.8cm,
      },
      conv axis,
      width=#1,
      height=#2,
    ]
#3
    \end{groupplot}
  \end{tikzpicture}
}

\newcommand{\AdjointConvergencePanel}[3]{%
  \begin{tikzpicture}
    \begin{axis}[
      conv axis,
      width=#1,
      height=#2,
      xlabel={Objective evaluations},
      ylabel={Objective function $J$},
      legend columns=1,
      legend style={at={(0.97,0.97)}, anchor=north east},
    ]
#3
    \end{axis}
  \end{tikzpicture}
}


==> Figures/htc_pgfplots_macros.tex <==
\pgfplotsset{
  htc axis/.style={
    xmin=0,
    xmax=60,
    xlabel={x [mm]},
    ylabel={h [W/m$^2$/K]},
    grid=major,
    major grid style={draw=gray!35, line width=0.35pt},
    tick align=outside,
    tick style={black, line width=0.5pt},
    line width=0.85pt,
    axis line style={black},
    title style={font=\normalsize, yshift=2pt},
    label style={font=\small},
    tick label style={font=\small},
    legend style={
      draw=gray!55,
      fill=white,
      fill opacity=0.96,
      text opacity=1,
      rounded corners=1pt,
      font=\footnotesize,
    },
    legend cell align=left,
    unbounded coords=discard,
  },
  htcCommonSeries/.style={
    solid,
    line width=1.15pt,
    mark=*,
    mark repeat=12,
    mark size=1.1pt,
    mark options={fill=white},
  },
  htcLegendLine/.style={
    solid,
    line width=1.15pt,
    mark=none,
  },
  htcColorGroundTruth/.style={color=black},
  htcColorAdjoint/.style={color=red!75!black},
  htcColorScratch/.style={color=blue!75!black},
  htcColorFT/.style={color=green!50!black},
  htcColorTL/.style={color=violet!80!black},
  htcColorTLGauss/.style={color=teal!70!black},
  htcColorNN/.style={color=orange!85!black},
  htcNoiseFree/.style={
    solid,
    mark=none,
  },
  htcNoiseFive/.style={
    dotted,
    mark=none,
  },
  htcNoiseTen/.style={
    dashed,
    mark=none,
  },
  htcGroundTruth/.style={
    htcCommonSeries,
    color=black,
    line width=1.3pt,
    mark options={draw=black, fill=white},
  },
  htcAdjoint/.style={
    htcCommonSeries,
    color=red!75!black,
    mark options={draw=red!75!black, fill=white},
  },
  htcScratch/.style={
    htcCommonSeries,
    color=blue!75!black,
    mark options={draw=blue!75!black, fill=white},
  },
  htcFT/.style={
    htcCommonSeries,
    color=green!50!black,
    mark options={draw=green!50!black, fill=white},
  },
  htcTL/.style={
    htcCommonSeries,
    color=violet!80!black,
    mark options={draw=violet!80!black, fill=white},
  },
  htcTLGauss/.style={
    htcCommonSeries,
    color=teal!70!black,
    mark options={draw=teal!70!black, fill=white},
  },
  htcNN/.style={
    htcCommonSeries,
    color=orange!85!black,
    mark options={draw=orange!85!black, fill=white},
  },
}

\newcommand{\HTCAddSeries}[5]{%
  \addplot+[
    #5,
  ] table[
    col sep=comma,
    x=xmm,
    y=val,
    restrict expr to domain={\thisrow{noise}}{#2:#2},
    restrict expr to domain={\thisrow{methodid}}{#3:#3},
  ] {#1};
  \addlegendentry{#4}
}

\newcommand{\HTCAddLegendItem}[2]{%
  \addlegendimage{#1}%
  \addlegendentry{#2}%
}

\newcommand{\HTCAddOverallSeries}[6]{%
  \addplot+[
    line width=1.25pt,
    #5,
    #6,
  ] table[
    col sep=comma,
    x=xmm,
    y=val,
    restrict expr to domain={\thisrow{noise}}{#2:#2},
    restrict expr to domain={\thisrow{methodid}}{#3:#3},
  ] {#1};
}

\newcommand{\HTCSinglePanel}[6]{%
  \begin{tikzpicture}
    \begin{axis}[
      htc axis,
      width=#1,
      height=#2,
      title={#3},
      ymin=#4,
      ymax=#5,
      legend columns=2,
      legend style={at={(0.98,0.98)}, anchor=north east},
    ]
#6
    \end{axis}
  \end{tikzpicture}
}

\newcommand{\HTCOverallLegend}[2]{%
  \begin{tikzpicture}
    \begin{axis}[
      hide axis,
      xmin=0,
      xmax=1,
      ymin=0,
      ymax=1,
      legend columns=#1,
      legend style={
        draw=gray!55,
        fill=white,
        fill opacity=0.96,
        text opacity=1,
        rounded corners=1pt,
        font=\footnotesize,
        /tikz/every even column/.append style={column sep=0.8em},
      },
    ]
#2
    \end{axis}
  \end{tikzpicture}
}

\newcommand{\HTCOverallPanel}[6]{%
  \begin{tikzpicture}
    \begin{groupplot}[
      group style={
        group size=3 by 1,
        horizontal sep=0.95cm,
      },
      htc axis,
      width=#1,
      height=#2,
      ymin=#3,
      ymax=#4,
      title style={font=\normalsize, yshift=1pt},
    ]
#6
    \end{groupplot}
  \end{tikzpicture}
}


==> Figures/results_representative_loss_histories.tex <==
\begin{figure}[!htbp]
  \centering
  \tikzset{external/export next=false}
  \begin{tikzpicture}
    \begin{groupplot}[
      group style={group size=2 by 2, horizontal sep=1.15cm, vertical sep=1.25cm},
      selected loss axis,
      width=0.455\linewidth,
      height=4.8cm,
    ]
      \nextgroupplot[title={Fixed Re: PWL, 5\% noise},xlabel={}]
      \CommonLossAddSeries{data/convergence/table8_pinn_common_loss.csv}{noise}{5}{0}{1}{0}{selectedTLTrain}
      \CommonLossAddSeries{data/convergence/table8_pinn_common_loss.csv}{noise}{5}{0}{1}{1}{selectedTLTest}

      \nextgroupplot[title={Fixed Re: NN estimator, 5\% noise},xlabel={},ylabel={},yticklabels={}]
      \CommonLossAddSeries{data/convergence/table8_pinn_common_loss.csv}{noise}{5}{1}{1}{0}{selectedTLTrain}
      \CommonLossAddSeries{data/convergence/table8_pinn_common_loss.csv}{noise}{5}{1}{1}{1}{selectedTLTest}

      \nextgroupplot[title={PWL PINN total loss, $\mathrm{Re}=10000$}]
      \CommonLossAddSeries{data/convergence/table10_pinn_common_loss.csv}{reynolds}{10000}{0}{1}{0}{selectedTLTrain}
      \CommonLossAddSeries{data/convergence/table10_pinn_common_loss.csv}{reynolds}{10000}{0}{1}{1}{selectedTLTest}

      \nextgroupplot[title={NN PINN total loss, $\mathrm{Re}=10000$},ylabel={},yticklabels={}]
      \CommonLossAddSeries{data/convergence/table10_pinn_common_loss.csv}{reynolds}{10000}{1}{1}{0}{selectedTLTrain}
      \CommonLossAddSeries{data/convergence/table10_pinn_common_loss.csv}{reynolds}{10000}{1}{1}{1}{selectedTLTest}
    \end{groupplot}
  \end{tikzpicture}

  \vspace{0.25em}
  {\footnotesize
  \begin{tabular}{@{}ll@{\qquad}ll@{}}
    \SelectedLegendLine{green!50!black,line width=1.1pt,solid} & Transfer train &
    \SelectedLegendLine{magenta!70!black,line width=1.1pt,densely dashed} & Transfer test
  \end{tabular}}
  \caption{Representative transferred-model PINN convergence histories for
  the two transfer pathways. The top row shows transfer from the noise-free
  model to the 5\%-noise target at $\mathrm{Re}=5000$; the bottom row shows
  Gaussian-source transfer to the 5\%-noise $\mathrm{Re}=10000$ target. Every
  corrected 1000-iteration checkpoint is retained. The total PINN loss shown is the sum
  of the PDE, four boundary-condition, initial-condition, and observation
  components.}
  \label{fig:results_representative_tl_loss}
\end{figure}


==> Figures/table9_gaussian_source.tex <==
\tikzexternaldisable
\definecolor{tableNineBlue}{HTML}{0072B2}

\pgfplotsset{
  table nine axis/.style={
    xmin=0,
    xmax=60,
    ymin=0,
    ymax=110,
    xtick={0,10,...,60},
    ytick={0,20,...,100},
    xlabel={$x$ [mm]},
    grid=major,
    major grid style={draw=gray!30, line width=0.3pt},
    tick align=outside,
    axis line style={black},
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small, yshift=1pt},
    unbounded coords=discard,
  },
  table nine reference/.style={
    black,
    solid,
    line width=1.35pt,
    mark=none,
  },
  table nine source/.style={
    tableNineBlue,
    dashdotted,
    line width=1.2pt,
    mark=none,
  },
}

\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=2 by 1, horizontal sep=1.15cm},
  table nine axis,
  width=0.46\textwidth,
  height=0.31\textwidth,
]

\nextgroupplot[
  title={(a) PWL representation},
  ylabel={HTC, $h$ [W\,m$^{-2}$\,K$^{-1}$]},
  legend to name=tableNineLegend,
  legend columns=2,
  legend cell align=left,
  legend style={
    draw=gray!55,
    fill=white,
    font=\scriptsize,
    /tikz/every even column/.append style={column sep=0.8em},
  },
]
\addlegendimage{table nine reference}
\addlegendentry{Reference}
\addlegendimage{table nine source}
\addlegendentry{PINN source}
\addplot[table nine source, forget plot]
  table[col sep=comma, x=x_mm, y=h_estimated_W_m2K]
  {data/table9_gaussian_source/pwl_source_native.csv};
\addplot[table nine reference, forget plot]
  table[col sep=comma, x=x_mm, y=h_reference_W_m2K]
  {data/table9_gaussian_source/pwl_source_native.csv};

\nextgroupplot[title={(b) NN-estimator representation}]
\addplot[table nine source]
  table[col sep=comma, x=x_mm, y=h_estimated_W_m2K]
  {data/table9_gaussian_source/nn_source_native.csv};
\addplot[table nine reference]
  table[col sep=comma, x=x_mm, y=h_reference_W_m2K]
  {data/table9_gaussian_source/nn_source_native.csv};

\end{groupplot}
\end{tikzpicture}

\vspace{0.4em}
\pgfplotslegendfromname{tableNineLegend}
\caption{Noise-free Gaussian source-profile reconstruction using the 1-s
sampling interval. The PWL and NN-estimator curves are plotted on their complete
200-point native grids.}
\label{fig:table9_gaussian_source_profiles}
\end{figure}

